HR-Agents: Using Multiple LLM-based Agents to Improve Q&A about Brazilian Labor Legislation

The Consolidation of Labor Laws (CLT) serves as the primary legal framework governing labor relations in Brazil, ensuring essential protections for workers. However, its complexity creates challenges for Human Resources (HR) professionals in navigating regulations and ensuring compliance. Traditional methods for addressing labor law inquiries often lead to inefficiencies, delays, and inconsistencies. To enhance the accuracy and efficiency of legal question-answering (Q&A), a multi-agent system powered by Large Language Models (LLMs) is introduced. This approach employs specialized agents to address distinct aspects of employment law while integrating Retrieval-Augmented Generation (RAG) to enhance contextual relevance. Implemented using CrewAI, the system enables cooperative agent interactions, ensuring response validation and reducing misinformation. The effectiveness of this framework is evaluated through a comparison with a baseline RAG pipeline utilizing a single LLM, using automated metrics such as BLEU, LLM-as-judge evaluations, and expert human assessments. Results indicate that the multi-agent approach improves response coherence and correctness, providing a more reliable and efficient solution for HR professionals. This study contributes to AI-driven legal assistance by demonstrating the potential of multi-agent LLM architectures in improving labor law compliance and streamlining HR operations.

==> sections/discussion.tex <==
\section{Discussion}
\label{s.discussion}



==> sections/related.tex <==
\section{Related works}
\label{s.related}

The widespread adoption of LLMs has enhanced automation, personalization, and efficiency in AI-driven interactions. However, their use in HR, particularly in labor law compliance, workplace policy interpretation, and employee relations, remains underexplored. 

Since HR-specific studies are limited, examining adjacent fields like customer service automation and multi-agent AI frameworks helps identify relevant methodologies. The following works contribute to designing intelligent conversational agents, validating AI responses, and fostering user trust, forming a foundation for LLM-based HR solutions.

A notable contribution in this area is CHOPS: Chat with Customer Profile Systems for Customer Service with LLMs \citep{shi2024chops}, which proposes a structured approach to refining LLM-generated responses. CHOPS integrates user databases with external systems, utilizing an "Execution-Verifier" framework to validate AI outputs. The study introduces the CPHOS dataset, which includes a QA validation framework, allowing systematic benchmarking of agent effectiveness. To optimize inference costs, CHOPS employs a Classifier-Executor-Verifier model that dynamically determines the necessity of API calls and reference retrieval, improving both response accuracy and computational efficiency.

Further expanding on modular agent architectures, AutoGen \citep{wu2023autogen} presents an open-source framework for designing LLM-based multi-agent systems capable of inter-agent communication. This framework facilitates the creation of customizable conversational agents, which can operate autonomously or in hybrid configurations, incorporating human supervision and external tool integration. By enabling collaborative workflows between specialized agents, AutoGen enhances the adaptability and scalability of AI-driven customer service solutions.

In domain-specific implementations, \citet{ngai2021intelligent} explore the impact of AI-driven conversational agents within e-commerce environments. Through a case study, the research demonstrates the effectiveness of intelligent virtual assistants in improving customer engagement, service efficiency, and response quality, reinforcing the potential of LLM-based solutions in industry-specific applications.

Beyond customer service, the role of multi-agent LLM frameworks has gained traction in AI research. \citet{qian2023communicative} proposes a role-based multi-agent system that simulates a software development team, with specialized agents. This structured methodology decomposes complex engineering tasks into sequential atomic subtasks, optimizing AI-driven collaboration. While primarily applied to software development, the underlying principles of agent specialization and coordination hold relevance for HR applications, particularly in structuring legal consultation workflows.

Addressing trust-building mechanisms in AI-driven services, \citet{wang2021trust} propose a comprehensive framework based on the Ability-Benevolence-Integrity (ABI) model, synthesizing multiple perspectives on AI trustworthiness. Their empirical analysis provides insights into designing conversational agents that prioritize transparency, reliability, and ethical considerations, which are essential for AI applications in legally sensitive domains like HR compliance and labor law consultation.

Research on LLM-based customer support has shown success in handling inquiries, optimizing workflows, and improving response accuracy. These advancements provide useful insights for LLM-based agents, but HR automation requires greater legal and contextual accuracy.

